The Ambiguity of Simplicity

A system's apparent simplicity depends on whether it is represented classically or quantally. This is not so surprising, as classical and quantum physics are descriptive frameworks built on different assumptions that capture, emphasize, and express different properties and mechanisms. What is surprising is that, as we demonstrate, simplicity is ambiguous: the relative simplicity between two systems can change sign when moving between classical and quantum descriptions. Thus, notions of absolute physical simplicity---minimal structure or memory---at best form a partial, not a total, order. This suggests that appeals to principles of physical simplicity, via Ockham's Razor or to the "elegance" of competing theories, may be fundamentally subjective, perhaps even beyond the purview of physics itself. It also raises challenging questions in model selection between classical and quantum descriptions. Fortunately, experiments are now beginning to probe measures of simplicity, creating the potential to directly test for ambiguity.

==> cmechabbrev.tex <==
% Abbreviations from CMPPSS:

\newcommand{\eM}     {\mbox{$\epsilon$-machine}\xspace}
\newcommand{\eMs}    {\mbox{$\epsilon$-machines}\xspace}
\newcommand{\EM}     {\mbox{$\epsilon$-Machine}\xspace}
\newcommand{\EMs}    {\mbox{$\epsilon$-Machines}\xspace}
\newcommand{\eT}     {\mbox{$\epsilon$-transducer}\xspace}
\newcommand{\eTs}    {\mbox{$\epsilon$-transducers}\xspace}
\newcommand{\ET}     {\mbox{$\epsilon$-Transducer}\xspace}
\newcommand{\ETs}    {\mbox{$\epsilon$-Transducers}\xspace}

% cryptic
\newcommand{\order}[1]{order\protect\nobreakdash-$#1$}
\newcommand{\Order}[1]{Order\protect\nobreakdash-$#1$}
\newcommand{\cryptic}[1]{$#1$\protect\nobreakdash-cryptic}
\newcommand{\Cryptic}[1]{$#1$\protect\nobreakdash-Cryptic}
\newcommand{\crypticity}[1]{$#1$\protect\nobreakdash-crypticity}
\newcommand{\Crypticity}[1]{$#1$\protect\nobreakdash-Crypticity}

% Processes and sequences

\newcommand{\Process}{\mathcal{P}}

\newcommand{\ProbMach}{\Prob_{\mathrm{M}}}
\newcommand{\Lmax}   { {L_{\mathrm{max}}}}
\newcommand{\MeasAlphabet}      {\mathcal{A}}
% Original symbol
%\newcommand{\MeasSymbol}   { {S} }
%\newcommand{\meassymbol}   { {s} }
% New symbol
\newcommand{\MeasSymbol}   { {X} }
\newcommand{\meassymbol}   { {x} }
\newcommand{\BiInfinity}        { \smash{\overleftrightarrow {\MeasSymbol}} }
\newcommand{\biinfinity}        { \smash{\overleftrightarrow {\meassymbol}} }
\newcommand{\Past}      { \smash{\overleftarrow {\MeasSymbol}} }
\newcommand{\past}      { \smash{\overleftarrow {\meassymbol}} }
\newcommand{\pastprime} { {\past}^{\prime}}
\newcommand{\Future}    { \smash{\overrightarrow{\MeasSymbol}} }
\newcommand{\future}    { \smash{\overrightarrow{\meassymbol}} }
\newcommand{\futureprime}       { \smash{\future^{\prime}} }
\newcommand{\PastPrime}     { \smash{\Past^{\prime}} }
\newcommand{\FuturePrime}       { \smash{\overrightarrow{\meassymbol}^\prime} }
\newcommand{\PastDblPrime}      { \smash{\overleftarrow{\meassymbol}^{\prime\prime}} }
\newcommand{\FutureDblPrime}{ \smash{\overrightarrow{\meassymbol}^{\prime\prime}} }
\newcommand{\pastL}     { \smash{\overleftarrow {\meassymbol}{}^L} }
\newcommand{\PastL}     { \smash{\overleftarrow {\MeasSymbol}{}^L} }
\newcommand{\PastLt}      { \smash{\overleftarrow {\MeasSymbol}_t^L} }
\newcommand{\PastLLessOne}{ \smash{\overleftarrow {\MeasSymbol}^{L-1}} }
\newcommand{\futureL}     { \smash{\overrightarrow{\meassymbol}{}^L} }
\newcommand{\FutureL}     { \smash{\overrightarrow{\MeasSymbol}{}^L} }
\newcommand{\FutureLt}    { \smash{\overrightarrow{\MeasSymbol}_t^L} }
\newcommand{\FutureLLessOne}{ \smash{\overrightarrow{\MeasSymbol}^{L-1}} }
\newcommand{\pastLprime}        { \smash{\overleftarrow {\meassymbol}^{L^\prime}} }
\newcommand{\futureLprime}      { \smash{\overrightarrow{\meassymbol}^{L^\prime}} }
\newcommand{\AllPasts}      { \smash{\overleftarrow{ {\rm {\bf \MeasSymbol}} } } }
\newcommand{\AllFutures}        { \smash{\overrightarrow{ {\rm {\bf \MeasSymbol}} } } }
\newcommand{\FutureSet} { \smash{\overrightarrow{\bf \MeasSymbol}} }

% Causal states and epsilon-machines
\newcommand{\CausalState}       { \mathcal{S} }
\newcommand{\CausalStatePrime}  { {\CausalState}^{\prime}}
\newcommand{\causalstate}       { \sigma }
\newcommand{\CausalStateSet}    { \boldsymbol{\CausalState} }
\newcommand{\AlternateState}    { \mathcal{R} }
\newcommand{\AlternateStatePrime}       { {\cal R}^{\prime} }
\newcommand{\alternatestate}    { \rho }
\newcommand{\alternatestateprime}       { {\rho^{\prime}} }
\newcommand{\AlternateStateSet} { \boldsymbol{\AlternateState} }
\newcommand{\PrescientState}    { \widehat{\AlternateState} }
\newcommand{\prescientstate}    { \widehat{\alternatestate} }
\newcommand{\PrescientStateSet} { \boldsymbol{\PrescientState}}
\newcommand{\CausalEquivalence} { {\sim}_{\epsilon} }
\newcommand{\CausalEquivalenceNot}      { {\not \sim}_{\epsilon}}

\newcommand{\NonCausalEquivalence}      { {\sim}_{\eta} }
\newcommand{\NextObservable}    { {\smash{\overrightarrow {\MeasSymbol}}^1} }
\newcommand{\LastObservable}    { {\smash{\overleftarrow {\MeasSymbol}}^1} }
%\newcommand{\Prob}             { {\rm P}}
\newcommand{\Prob}      {\Pr} % use standard command
\newcommand{\ProbAnd}   { {,\;} }
\newcommand{\LLimit}    { {L \rightarrow \infty}}
\newcommand{\Cmu}               {C_\mu}
\newcommand{\hmu}               {h_\mu}
\newcommand{\EE}                {{\bf E}}
\newcommand{\TI}                {{\bf T}}
\newcommand{\SyncI}        {{\bf S}}
\newcommand{\Measurable}{{\bf \mu}}

% Process Crypticity
\newcommand{\PC}                {\chi}

% Causal Irreversibility
\newcommand{\CI}                {\Xi}
\newcommand{\ReverseMap}        {r}
\newcommand{\ForwardMap}        {f}

% Abbreviations from IB:
% None that aren't already in CMPPSS

% Abbreviations from Extensive Estimation:
\newcommand{\EstCausalState}    {\widehat{\CausalState}}
\newcommand{\estcausalstate}    {\widehat{\causalstate}}
\newcommand{\EstCausalStateSet} {\boldsymbol{\EstCausalState}}
\newcommand{\EstCausalFunc}     {\widehat{\epsilon}}
\newcommand{\EstCmu}            {\widehat{\Cmu}}
\newcommand{\PastLOne}  {{\Past}^{L+1}}
\newcommand{\pastLOne}  {{\past}^{L+1}}

% Abbreviations from $\epsilon$-Transducers:
\newcommand{\InAlphabet}        { \mathcal{A}}
\newcommand{\insymbol}          { a}
\newcommand{\OutAlphabet}       { \mathcal{B}}
\newcommand{\outsymbol}         { b}
\newcommand{\InputSimple}       { X}
\newcommand{\inputsimple}       { x}
\newcommand{\BottleneckVar}     {\tilde{\InputSimple}}
\newcommand{\bottleneckvar}     {\tilde{\inputsimple}}
\newcommand{\InputSpace}        { \mathbf{\InputSimple}}
\newcommand{\InputBi}   { \overleftrightarrow {\InputSimple} }
\newcommand{\inputbi}   { \overleftrightarrow {\inputsimple} }
\newcommand{\InputPast} { \overleftarrow {\InputSimple} }
\newcommand{\inputpast} { \overleftarrow {\inputsimple} }
\newcommand{\InputFuture}       { \overrightarrow {\InputSimple} }
\newcommand{\inputfuture}       { \overrightarrow {\inputsimple} }
\newcommand{\NextInput} { {{\InputFuture}^{1}}}
\newcommand{\NextOutput}        { {\OutputFuture}^{1}}
\newcommand{\OutputSimple}      { Y}
\newcommand{\outputsimple}      { y}
\newcommand{\OutputSpace}       { \mathbf{\OutputSimple}}
\newcommand{\OutputBi}  { \overleftrightarrow{\OutputSimple} }
\newcommand{\outputbi}  { \overleftrightarrow{\outputsimple} }
\newcommand{\OutputPast}        { \overleftarrow{\OutputSimple} }
\newcommand{\outputpast}        { \overleftarrow{\outputsimple} }
\newcommand{\OutputFuture}      { \overrightarrow{\OutputSimple} }
\newcommand{\outputfuture}      { \overrightarrow{\outputsimple} }
\newcommand{\OutputL}   { {\OutputFuture}^L}
\newcommand{\outputL}   { {\outputfuture}^L}
\newcommand{\InputLLessOne}     { {\InputFuture}^{L-1}}
\newcommand{\inputLlessone}     { {\inputufutre}^{L-1}}
\newcommand{\OutputPastLLessOne}        {{\OutputPast}^{L-1}_{-1}}
\newcommand{\outputpastLlessone}        {{\outputpast}^{L-1}}
\newcommand{\OutputPastLessOne} {{\OutputPast}_{-1}}
\newcommand{\outputpastlessone} {{\outputpast}_{-1}}
\newcommand{\OutputPastL}       {{\OutputPast}^{L}}
\newcommand{\OutputLPlusOne}    { {\OutputFuture}^{L+1}}
\newcommand{\outputLplusone}    { {\outputfutre}^{L+1}}
\newcommand{\InputPastL}        {{\InputPast}^{L}}
\newcommand{\inputpastL}        {{\inputpast}^{L}}
\newcommand{\JointPast} {{(\InputPast,\OutputPast)}}
\newcommand{\jointpast} {{(\inputpast,\outputpast)}}
\newcommand{\jointpastone}      {{(\inputpast_1,\outputpast_1)}}
\newcommand{\jointpasttwo}      {{(\inputpast_2,\outputpast_2)}}
\newcommand{\jointpastprime} {{({\inputpast}^{\prime},{\outputpast}^{\prime})}}
\newcommand{\NextJoint} {{(\NextInput,\NextOutput)}}
\newcommand{\nextjoint} {{(\insymbol,\outsymbol)}}
\newcommand{\AllInputPasts}     { { \overleftarrow {\rm \InputSpace}}}
\newcommand{\AllOutputPasts}    { {\overleftarrow {\rm \OutputSpace}}}
\newcommand{\DetCausalState}    { {{\cal S}_D }}
\newcommand{\detcausalstate}    { {{\sigma}_D} }
\newcommand{\DetCausalStateSet} { \boldsymbol{{\CausalState}_D}}
\newcommand{\DetCausalEquivalence}      { {\sim}_{{\epsilon}_{D}}}
\newcommand{\PrescientEquivalence}      { {\sim}_{\widehat{\eta}}}
\newcommand{\FeedbackCausalState}       { \mathcal{F}}
\newcommand{\feedbackcausalstate}       { \phi}
\newcommand{\FeedbackCausalStateSet}    { \mathbf{\FeedbackCausalState}}
\newcommand{\JointCausalState}          { \mathcal{J}}
\newcommand{\JointCausalStateSet}       { \mathbf{\JointCausalState}}
\newcommand{\UtilityFunctional} { {\mathcal{L}}}
\newcommand{\NatureState}       { {\Omega}}
\newcommand{\naturestate}       { {\omega}}
\newcommand{\NatureStateSpace}  { {\mathbf{\NatureState}}}
\newcommand{\AnAction}  { {A}}
\newcommand{\anaction}  { {a}}
\newcommand{\ActionSpace}       { {\mathbf{\AnAction}}}

% Abbreviations from RURO:
\newcommand{\InfoGain}[2] { \mathcal{D} \left( {#1} || {#2} \right) }

% Abbreviations from Upper Bound:
\newcommand{\lcm}       {{\rm lcm}}
% Double-check that this isn't in the math set already!

% Abbreviations from Emergence in Space
\newcommand{\ProcessAlphabet}   {\MeasAlphabet}
\newcommand{\ProbEst}                   { {\widehat{\Prob}_N}}
\newcommand{\STRegion}                  { {\mathrm K}}
\newcommand{\STRegionVariable}          { K}
\newcommand{\stregionvariable}          { k}
\newcommand{\GlobalPast}                { \overleftarrow{G}}
\newcommand{\globalpast}                { \overleftarrow{g}}
\newcommand{\GlobalFuture}              { \overrightarrow{G}}
\newcommand{\globalfuture}              { \overrightarrow{g}}
\newcommand{\GlobalState}               { \mathcal{G}}
\newcommand{\globalstate}               { \gamma}
\newcommand{\GlobalStateSet}            { {\mathbf \GlobalState}}
\newcommand{\LocalPast}                 { \overleftarrow{L}}
\newcommand{\localpast}                 { \overleftarrow{l}}
\newcommand{\AllLocalPasts}             { \mathbf{\LocalPast}}
\newcommand{\LocalPastRegion}           { \overleftarrow{\mathrm L}}
\newcommand{\LocalFuture}               { \overrightarrow{L}}
\newcommand{\localfuture}               { \overrightarrow{l}}
\newcommand{\LocalFutureRegion}         { \overrightarrow{\mathrm L}}
\newcommand{\LocalState}                { \mathcal{L}}
\newcommand{\localstate}                { \lambda}
\newcommand{\LocalStateSet}             { {\mathbf \LocalState}}
\newcommand{\PatchPast}                 { \overleftarrow{P}}
\newcommand{\patchpast}                 { \overleftarrow{p}}
\newcommand{\PatchPastRegion}           { \overleftarrow{\mathrm P}}
\newcommand{\PatchFuture}               { \overrightarrow{P}}
\newcommand{\patchfuture}               { \overrightarrow{p}}
\newcommand{\PatchFutureRegion}         { \overrightarrow{\mathrm P}}
\newcommand{\PatchState}                { \mathcal{P}}
\newcommand{\patchstate}                { \pi}
\newcommand{\PatchStateSet}             { {\mathbf \PatchState}}
\newcommand{\LocalStatesInPatch}        {\vec{\LocalState}}
\newcommand{\localstatesinpatch}        {\vec{\localstate}}
\newcommand{\PointInstantX}             { {\mathbf x}}
% Galles's original LaTeX for the cond. indep. symbol follows:
\newcommand{\compos}{\mbox{$~\underline{~\parallel~}~$}}
\newcommand{\ncompos}{\not\hspace{-.15in}\compos}
\newcommand{\indep}                     { \rotatebox{90}{$\models$}}
\newcommand{\nindep}    {\not\hspace{-.05in}\indep}
\newcommand{\LocalEE}   {{\EE}^{loc}}
\newcommand{\EEDensity} {\overline{\LocalEE}}
\newcommand{\LocalCmu}  {{\Cmu}^{loc}}
\newcommand{\CmuDensity}        {\overline{\LocalCmu}}

%%%%%%%%%%% added by sasa
\newcommand{\FinPast}[1]        { \overleftarrow {\MeasSymbol} \stackrel{{#1}}{}}
\newcommand{\finpast}[1]        { \overleftarrow {\meassymbol}  \stackrel{{#1}}{}}
\newcommand{\FinFuture}[1]              { \overrightarrow{\MeasSymbol} \stackrel{{#1}}{}}
\newcommand{\finfuture}[1]              { \overrightarrow{\meassymbol} \stackrel{{#1}}{}}

\newcommand{\Partition} { \AlternateState }
\newcommand{\partitionstate}    { \alternatestate }
\newcommand{\PartitionSet}      { \AlternateStateSet }
\newcommand{\Fdet}   { F_{\rm det} }

\newcommand{\Dkl}[2] { D_{\rm KL} \left( {#1} || {#2} \right) }

\newcommand{\Period}    {p}

% To take into account time direction
\newcommand{\forward}{+}
\newcommand{\reverse}{-}
%\newcommand{\forwardreverse}{\:\!\diamond} % \pm
\newcommand{\forwardreverse}{\pm} % \pm
\newcommand{\FutureProcess}     { {\Process}^{\forward} }
\newcommand{\PastProcess}       { {\Process}^{\reverse} }
\newcommand{\FutureCausalState} { {\CausalState}^{\forward} }
\newcommand{\futurecausalstate} { \sigma^{\forward} }
\newcommand{\altfuturecausalstate}      { \sigma^{\forward\prime} }
\newcommand{\PastCausalState}   { {\CausalState}^{\reverse} }
\newcommand{\pastcausalstate}   { \sigma^{\reverse} }
\newcommand{\BiCausalState}             { {\CausalState}^{\forwardreverse} }
\newcommand{\bicausalstate}             { {\sigma}^{\forwardreverse} }
\newcommand{\FutureCausalStateSet}      { {\CausalStateSet}^{\forward} }
\newcommand{\PastCausalStateSet}        { {\CausalStateSet}^{\reverse} }
\newcommand{\BiCausalStateSet}  { {\CausalStateSet}^{\forwardreverse} }
\newcommand{\eMachine}  { M }
\newcommand{\FutureEM}  { {\eMachine}^{\forward} }
\newcommand{\PastEM}    { {\eMachine}^{\reverse} }
\newcommand{\BiEM}              { {\eMachine}^{\forwardreverse} }
\newcommand{\BiEquiv}   { {\sim}^{\forwardreverse} }
\newcommand{\Futurehmu} { h_\mu^{\forward} }
\newcommand{\Pasthmu}   { h_\mu^{\reverse} }
\newcommand{\FutureCmu} { C_\mu^{\forward} }
\newcommand{\PastCmu}   { C_\mu^{\reverse} }
\newcommand{\BiCmu}             { C_\mu^{\forwardreverse} }
\newcommand{\FutureEps} { \epsilon^{\forward} }
\newcommand{\PastEps}   { \epsilon^{\reverse} }
\newcommand{\BiEps}     { \epsilon^{\forwardreverse} }
\newcommand{\FutureSim} { \sim^{\forward} }
\newcommand{\PastSim}   { \sim^{\reverse} }
\newcommand{\FuturePC}  {\PC^{\forward}}
\newcommand{\PastPC}            {\PC^{\reverse}}
\newcommand{\BiPC}      {\PC^{\forwardreverse}}

% Used arrows for awhile, more or less confusing?
%\newcommand{\FutureCausalState}        { \overrightarrow{\CausalState} }
%\newcommand{\PastCausalState}  { \overleftarrow{\CausalState} }
%\newcommand{\eMachine} { M }
%\newcommand{\FutureEM} { \overrightarrow{\eMachine} }
%\newcommand{\PastEM}   { \overleftarrow{\eMachine} }
%\newcommand{\FutureCmu}        { \overrightarrow{\Cmu} }
%\newcommand{\PastCmu}  { \overleftarrow{\Cmu} }

%% time-reversing and mixed state presentation operators
\newcommand{\TR}{\mathcal{T}}
\newcommand{\MSP}{\mathcal{U}}
\newcommand{\one}{\mathbf{1}}

%% added for RURO2
%% Note that it will always be typesett in math mode.
%% Example usage:
%%    The 3-block entropy is \BE[t]{3}.
%%    The 3-block-state entropy from $t=0$ is $\BSE{3}$.
%%
%% The optional argument specifies the start time, defaulting to t=0.
%% The mandatory argument specifies the length of the block (not the stop time).
\newcommand{\lastindex}[2]{
  \edef\tempa{0}
  \edef\tempb{#2}
  \ifx\tempa\tempb
    % if the length is 0, then the final time equals the start time
    \edef\tempc{#1}
  \else
    % if the start time is different from zero, then we show the sum
    \edef\tempa{0}
    \edef\tempb{#1}
    \ifx\tempa\tempb
      \edef\tempc{#2}
    \else
      \edef\tempc{#1+#2}
    \fi
  \fi
  \tempc
}
\newcommand{\BE}[2][0]{
  \ensuremath{H[\MeasSymbol_{#1}^{#2}]}
}
\newcommand{\BSE}[2][0]{
  \ensuremath{H[\MeasSymbol_{#1}^{#2},\CausalState_{\lastindex{#1}{#2}}]}%
}
\newcommand{\SBE}[2][0]{
  \ensuremath{H[\CausalState_{#1},\MeasSymbol_{#1}^{#2}]}
}
\newcommand{\SBSE}[2][0]{
  \ensuremath{H[\CausalState_{#1},\MeasSymbol_{#1}^{#2},
                \CausalState_{\lastindex{#1}{#2}}]}
}
\newcommand{\AltSBE}[2][0]{
  \ensuremath{H[\AlternateState_{#1},\MeasSymbol_{#1}^{#2}]}
}
\newcommand{\AltBSE}[2][0]{
  \ensuremath{H[\MeasSymbol_{#1}^{#2},\AlternateState_{\lastindex{#1}{#2}}]}
}
\newcommand{\AltSBSE}[2][0]{
  \ensuremath{H[\AlternateState_{#1},\MeasSymbol_{#1}^{#2},
                \AlternateState_{\lastindex{#1}{#2}}]}
}

\newcommand{\GI}{\ensuremath{\varphi}\xspace}
\newcommand{\OI}{\ensuremath{\zeta}\xspace}
% cryptic, gauge, oracular, Markov, and synchronization
\newcommand{\COrder}{\ensuremath{k_{\PC}}\xspace}
\newcommand{\GOrder}{\ensuremath{k_{\GI}}\xspace}
\newcommand{\OOrder}{\ensuremath{k_{\OI}}\xspace}
\newcommand{\MOrder}{\ensuremath{R}\xspace}
\newcommand{\SOrder}{\ensuremath{k_{\SI}}\xspace}


%% Added to standardize the order of causal states
%% Example usage:
%%    $\BiCmu = H[\CSjoint] = H[\CSjoint[,]]$
%%    $\EE = I[\CSjoint[:]] = I[\CSjoint[;]]$
\newcommand{\CSjoint}[1][,]{
   \edef\tempa{:}
   \edef\tempb{#1}
   \ifx\tempa\tempb
      % arg1 was a colon, insert a small negative space
      \ensuremath{\FutureCausalState\!#1\PastCausalState}
   \else
      % arg1 was not a colon, usually a comma or semicolon
      \ensuremath{\FutureCausalState#1\PastCausalState}
   \fi
}
\newcommand{\CSjointKL}[3][,]{
   \edef\tempa{:}
   \edef\tempb{#1}
   \ifx\tempa\tempb
      % arg1 was a colon, insert a small negative space
      \ensuremath{\FutureCausalState_{#2}\!#1\PastCausalState_{#3}}
   \else
      % arg1 was not a colon, usually a comma or semicolon
      \ensuremath{\FutureCausalState_{#2}#1\PastCausalState_{#3}}
   \fi
}


%% (cje)
%% Provide a command \ifpm which is true when \pm
%% is meant to be understood as "+ or -", opposed
%% to "bidirectional". This differs from the usage
%% in TBA.  Essentially, if \forwardreverse is defined
%% as something different, perhaps a \diamond, then
%% we are free to interpret \pm as "+ or -".
\newif\ifpm
\edef\tempa{\forwardreverse}
\edef\tempb{\pm}
\ifx\tempa\tempb
   \pmfalse
\else
   \pmtrue
\fi


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Metric quantities of information generation, eg anatomy of a bit

\newcommand{\metric}[1] {\ensuremath{#1_\mu}\xspace}

\renewcommand{\hmu}{\metric{h}}
\newcommand{\rhomu}{\metric{\rho}}
\newcommand{\rmu}{\metric{r}}
\newcommand{\bmu}{\metric{b}}
\newcommand{\qmu}{\metric{q}}
\newcommand{\wmu}{\metric{w}}
\newcommand{\imu}{\metric{i}}
\newcommand{\sigmamu}{\metric{\sigma}}

\newcommand{\himc}{\ensuremath{h_{imc}}\xspace}
\newcommand{\pee}{\ensuremath{pee}\xspace} % parallel edge entropy

\newcommand{\ExE}[1] {\ensuremath{\EE_{#1}}\xspace}

\newcommand{\EER}{\ExE{R}}
\newcommand{\EEB}{\ExE{B}}
\newcommand{\EEQ}{\ExE{Q}}
\newcommand{\EEW}{\ExE{W}}
\newcommand{\EI}{\mathbf{I}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Time series, using the python-esque notation

\newcommand{\MS} [2] {\ensuremath{\MeasSymbol_{#1:#2}}\xspace}
\newcommand{\ms} [2] {\ensuremath{\meassymbol_{#1:#2}}\xspace}

\renewcommand{\Past}       {\MS{}{0}}
\newcommand{\Present}      {\ensuremath{\MeasSymbol_{0}}\xspace}
\renewcommand{\Future}     {\MS{0}{}}
\newcommand{\LPresent} [1] {\MS{0}{#1}}
\newcommand{\LFuture}  [1] {\MS{#1}{}}

\renewcommand{\past}       {\ms{}{0}}
\newcommand{\present}      {\ensuremath{\meassymbol_{0}}\xspace}
\renewcommand{\future}     {\ms{0}{}}
\newcommand{\lpresent} [1] {\ms{0}{#1}}
\newcommand{\lfuture}  [1] {\ms{#1}{}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Causal states

\newcommand{\FCS}{\CausalState^\forward\xspace}
\newcommand{\RCS}{\CausalState^\reverse\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Others

\newcommand{\half}{\ensuremath{\nicefrac{1}{2}}}

\newcommand{\Language} {\ensuremath{\mathcal{L}}\xspace}
\newcommand{\Lsync} {\Language_{\mathrm{sync}}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% mathclap, in case someone doesn't have mathtools

% TUGboat, Volume 0 (2001), No. 0
% http://math.arizona.edu/~aprl/publications/mathclap/perlis_mathclap_24Jun2003.pdf
% For comparison, here are the existing overlap macros:
% \def\llap#1{\hbox to 0pt{\hss#1}}
% \def\rlap#1{\hbox to 0pt{#1\hss}}
%
% These are provided by mathtools
%
\ifcsname mathclap\endcsname
  \relax
\else
  \def\clap#1{\hbox to 0pt{\hss#1\hss}}
  \def\mathllap{\mathpalette\mathllapinternal}
  \def\mathrlap{\mathpalette\mathrlapinternal}
  \def\mathclap{\mathpalette\mathclapinternal}
  \def\mathllapinternal#1#2{%
    \llap{$\mathsurround=0pt#1{#2}$}}
  \def\mathrlapinternal#1#2{%
    \rlap{$\mathsurround=0pt#1{#2}$}}
  \def\mathclapinternal#1#2{%
    \clap{$\mathsurround=0pt#1{#2}$}}
\fi


==> infotheory.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Information theory macros

\def \mid {~\middle|~}

% functions
\newcommand{\op}  [2]   {\ensuremath{\operatorname{#1}\left[#2\right]}\xspace}

\renewcommand{\H} [1]   {\op{H}{#1}}
\newcommand{\I}   [1]   {\op{I}{#1}}
\newcommand{\T}   [1]   {\op{T}{#1}}
\newcommand{\R}   [1]   {\op{R}{#1}}
\newcommand{\B}   [1]   {\op{B}{#1}}
\newcommand{\K}   [1]   {\op{K}{#1}}

\newcommand{\TE}  [2]   {\ensuremath{\operatorname{T}_{#1\rightarrow#2}}\xspace}
\newcommand{\CE}  [3]   {\ensuremath{\operatorname{\mathcal{C}}_{#1\rightarrow#2|#3}}\xspace}

% operators on random variables
\newcommand{\meet}      {\curlywedge}
\newcommand{\join}      {\curlyvee}
\newcommand{\iless}     {\preceq}
\newcommand{\imore}     {\succeq}
\newcommand{\ieq}       {\cong}
\newcommand{\mss}       {\downrightarrow}

